Realizable Continuous-Space Shields for Safe Reinforcement Learning

While Deep Reinforcement Learning (DRL) has achieved remarkable success across various domains, it remains vulnerable to occasional catastrophic failures without additional safeguards. An effective solution to prevent these failures is to use a shield that validates and adjusts the agent's actions to ensure compliance with a provided set of safety specifications. For real-world robotic domains, it is essential to define safety specifications over continuous state and action spaces to accurately account for system dynamics and compute new actions that minimally deviate from the agent's original decision. In this paper, we present the first shielding approach specifically designed to ensure the satisfaction of safety requirements in continuous state and action spaces, making it suitable for practical robotic applications. Our method builds upon realizability, an essential property that confirms the shield will always be able to generate a safe action for any state in the environment. We formally prove that realizability can be verified for stateful shields, enabling the incorporation of non-Markovian safety requirements, such as loop avoidance. Finally, we demonstrate the effectiveness of our approach in ensuring safety without compromising the policy's success rate by applying it to a navigation problem and a multi-agent particle environment.

==> appendices/liveness-extended.tex <==
\subsection{Encoding Non-Markovian Requirements}
\label{sec:app:liveness-requirements}

LTLt, \cite{rodriguez2023boolean} is a specification language expressive enoough to reason about both time and data.
%
Moreover, using precise specifications of dynamics that the domain holds (essentially, Thm.~\ref{th:method:decidable}), in Ex.~\ref{ex:nonMarkovian} we showed that we can also enconde non-markovian properties that contain data.

\begin{example} \label{ex:properties}
    The following is a simplified encoding of the queues used in Sec.~\ref{sec:caseStudy}.
    
    Consider the only parameter to check is that a visited region $\text{reg} \in R$ in the arena is not visited for the next $k$ timesteps, then, we encode this property as follows: for all $\text{reg} \in R$, it holds that $\square [(x,y) \in \text{reg} \rightarrow \diamond_{[1,k]} (x,y) \notin \text{reg}]$, provided that the system cannot play to avoid that $(x,y) \in \text{reg}$ eventually happens (i.e., for all $\text{reg} \in R$, it also holds that $\diamond (x,y) \in \text{reg}$.
     
\end{example}

However, certification of such realizability (or unrealizability) is difficult to interpret for the designers, because it captures an explosion of combination of environment and system dynamics.

\begin{example}
    We attach in the supplementary zip a \texttt{dotfiles.org} with several graphs in \texttt{dotgraph} format to represent the strategies of the shields as automata\footnote{We also show the encoding in LTLt, the realizability result and the abstraction for Strix \cite{meyer18explicit}, which is the tool we used for realizability checking. Note that we are using Boolean abstractions as suggested by \cite{rodriguez2023boolean}. }. 
    %
    These show how very simple non-markovian specifications like the ones in Ex.~\ref{ex:properties} very quickly become not easy to explain.
    %
    \texttt{Shield(1,1)} encodes a single (temporaly) forbidden region with a single timestep horizon.
    %
   \texttt{Shield(2,1)} encodes a single forbidden region with a two timestep horizon.   
    %
   \texttt{Shield(3,1)} encodes a single forbidden region with a three timestep horizon.
    %
    We can see it that this size only increases linearly.
    %
    However, we have to add another dimension: more (temporaly) forbidden regions.
    %
    \texttt{Shield(1,2)} encodes a single (temporaly) forbidden region with a single timestep horizon.
    %
    \texttt{Shield(2,3)} encodes a single (temporaly) forbidden region with a two timestep horizon.
    %
    Note that this interpretation complexity grows exponentially (see figures for \texttt{Shield(1,1)}, \texttt{Shield(1,2)} and \texttt{Shield(2,2)} at the end of the appendices), but also note that realizability checking procedure's running time remains in seconds.
\end{example}

This suggests that like real-life non-markovian LTLt properties need to be defined encoded different way.
%
Therefore, in this paper we propose
shields that model non-markovian specifications, but all of them encoded as markovian specifications for the safety properties \textbf{plus} a stateful (thus, finite) memory that we called \textit{history} $H$ in Sec.~\ref{sec:method}. Since $H$ is stateful, decidability of this method is not compromised.
%
It is very important to note that $H$ has to hold certain properties depending on the domain of the problem:
%
\begin{itemize}
    \item Certain elements $h \in H$ cannot be followed by other $h'$. For instance, if the robot is region $x \in [0,10], y \in [0,10]$ in $h$ of position $i$, it cannot be in $x \in [800,900], y \in [800,900]$ in $h'$ of position $i+1$.
    \item The last $h$ in $H$ represents exactly the combination of the constraints that the previous state 
    $(x,y,r)$ satisfied and the constraints that previous movement $(a^0,a^1)$ satisfied. It is easy to see that the amount of combinations here is finite.
    \item It is not possible that, given arbitrary $h, h' \in H$, $h=h'$, which means that elements in $H$ cannot be repeated.
    \item Entries are related throughout time: i.e., if $h \in H$ appears in position $i$ in timestep $k$, it will be in position $i-1$ in timestep $k+1$.
\end{itemize}
%
Note again that these properties rely completely in the domain of the problem.

Then, if we guarantee these assumptions of the environment, we can specify the properties of the system in a straightforward manner: in every timestep, hold safety properties (inherently markovian) plus do not allow the output $o$ to be such that $o\in h$, for every $h \in H$.
%
This way, we can build a lightweight\footnote{In the sense that it will have way less states and thus will be easier to interpret.} shield that conform to the guarantees, whereas we delegate the assumptions to some other checker (which can be a synthetised model of the environment or any other \textbf{verified} program).
%
This yields extremely simple shields with more or less states that depend on the safety specifications and not the combinations of the non-markovian specifications.

In general, we can formally express this in the LTL synthesis notation as follows:

\begin{theorem}
\label{th:method:nonMarkov}

If a non-markovian specification $\varphi$ is realizable using stateful memory as an environment variable, then the property $\varphi'$ that encoding such memory as bounded-liveness in the side of the system is also realizable.
\end{theorem}

\begin{proof}
    
The proof sketch goes as follows: $\varphi$ is an over-approximation of the power of the environment in which we allow it to choose freely the values for $H$ in each timestep, and then we weaken this freedom by the properties like the aforementioned ones (e.g., no repeated element). Since $\varphi$ is an over-approximation of the power of the environment and it is realizable, then the version $\varphi'$
in which this power is not over-approximated is also necessarily realizable.

\end{proof}

\subsection{Figures of Shields} \label{subsec:figures}

We show below the strategies computed from three non-markovian specifications of Ex.~\ref{ex:nonMarkovian}.
%
The idea is to see how quickly they get difficult to interpret.

\begin{figure}[]
\centering
\includegraphics[width=0.3\linewidth]{images/mealy1.png} 
% \minipage{0.48\linewidth}
%     \includegraphics[width=\linewidth]{example-image-a} 
% \endminipage \hfill
% \minipage{0.48\linewidth}
%     \includegraphics[width=\linewidth]{example-image-b} 
% \endminipage
\caption{\texttt{Shield(1,1)}.}

\end{figure}


\begin{figure}[]
\centering
\includegraphics[width=1.0\linewidth]{images/mealy2.png} 
% \minipage{0.48\linewidth}
%     \includegraphics[width=\linewidth]{example-image-a} 
% \endminipage \hfill
% \minipage{0.48\linewidth}
%     \includegraphics[width=\linewidth]{example-image-b} 
% \endminipage
\caption{\texttt{Shield(1,2)}.}

\end{figure}

\begin{figure}[]
\centering
\includegraphics[width=1.0\linewidth]{images/mealy3.png} 
% \minipage{0.48\linewidth}
%     \includegraphics[width=\linewidth]{example-image-a} 
% \endminipage \hfill
% \minipage{0.48\linewidth}
%     \includegraphics[width=\linewidth]{example-image-b} 
% \endminipage
\caption{\texttt{Shield(2,2)}.}

\end{figure}


==> appendices/reproducibility.tex <==
\section*{Reproducibility Checklist}

This paper
\begin{itemize}
\item Includes a conceptual outline and/or pseudocode description of AI methods introduced (\textbf{yes})
\item Clearly delineates statements that are opinions, hypotheses, and speculations from objective facts and results (\textbf{yes})
\item Provides well-marked pedagogical references for less-familiar readers to gain the background necessary to replicate the paper (\textbf{yes})
\end{itemize}

Does this paper make theoretical contributions? (\textbf{yes})
If yes, please complete the list below.

\begin{itemize}
\item All assumptions and restrictions are stated clearly and formally. (\textbf{yes})
\item All novel claims are stated formally (e.g., in theorem statements). (\textbf{yes})
\item Proofs of all novel claims are included. (\textbf{yes})
\item Proof sketches or intuitions are given for complex and/or novel results. (\textbf{yes})
\item Appropriate citations to theoretical tools used are given. (\textbf{yes})
\item All theoretical claims are demonstrated empirically to hold. (\textbf{yes})
\item All experimental code used to eliminate or disprove claims are included. (\textbf{no})
\end{itemize} 

Does this paper rely on one or more datasets? (\textbf{no}) \\

Does this paper include computational experiments? (\textbf{yes})
If yes, please complete the list below.

\begin{itemize}
\item Any code required for pre-processing data is included in the appendix. (\textbf{no})
\item All source code required for conducting and analyzing the experiments is included in a code appendix. (\textbf{partial})
\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (\textbf{yes})
\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (\textbf{partial})
\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (\textbf{partial})
\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names, and versions of relevant software libraries and frameworks. (\textbf{yes})
\item This paper formally describes the evaluation metrics used and explains the motivation for choosing these metrics. (\textbf{yes})
\item This paper states the number of algorithm runs used to compute each reported result. (\textbf{yes})
\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (\textbf{yes})
\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed rank). (\textbf{partial})
\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (\textbf{partial})
\item This paper states the number and range of values tried per (hyper-) parameter during the development of the paper, along with the criterion used for selecting the final parameter setting. (\textbf{partial})
\end{itemize}

==> appendices/safety-extended.tex <==
\section{LTLt Details}

Since, due to space limitations, we could not formally explain two intuitions on how to use LTL modulo theories of \cite{rodriguez2023boolean} for our solution, we now detail them. In addition, the formal encoding of the requirements is available in the supplementary material; \textit{dotfiles.org} contains the specification in LTL, while the Python encoding is available in \textit{shield.py}.

\subsection{Relating Timesteps}
\label{sec:app:safety-requirements}

An essential observation used for this paper is that, using continuous domains with no uncertainty, we can usually \textit{anticipate} the dangerous movement of the system, because each valuation of $(a^0, a^1)$ in state $(x,y,r)$ induces a very precise next state.
%
This allows us to specify all the desired properties in decidable fragments of LTLt.

We capture this intuition more formally as follows: 

\begin{theorem}
\label{th:method:decidable}
Given a variable $v$ in $\varphi$, if the following conditions hold:
\begin{itemize}
    \item Valuation of $v$ in a future timestep $k_{\text{future}}$ can be fully inferred from a valuation in a previous step $k_{\text{past}} < k_{\text{future}}$; 
    \item and $v$ in $k_{\text{past}}$ only relates to variables in $k_{\text{past}}$ and $v$ in $k_{\text{future}}$ only relates to variables in $k_{\text{future}}$
\end{itemize}

Then every property expressed using $\lhd$ can also be expressed in an non-cross-state (NCS) formula.
\end{theorem}

\begin{proof}

The proof sketch goes as follows: Given the conditions on $v$ presented in the theorem, we can rewrite any formula containing $\lhd v$; concretely, 
%
$\lhd v$ can be replaced with a formula $\psi(v_{k_{\text{past}}})$ that only depends on the valuation of $v$ and other variables in the previous timestep $k_{\text{past}}$.
%
This is possible because the valuation of $v$ in the future timestep $k_{\text{future}}$ can be fully determined from the valuation in the previous timestep $k_{\text{past}}$.
By applying this rewriting, any formula containing $\lhd v$ can be transformed into an NCS formula that does not cross state boundaries. This is because the future state information is fully captured in the formula $\psi(v_{k_{\text{past}}})$, which only depends on the previous state.
    
\end{proof}

==> sections/introduction_dpr.tex <==

\section{Introduction}
\label{sec:introduction} 

Deep Reinforcement Learning (DRL) has achieved impressive results in a wide range of fields, demonstrating its potential to solve complex problems that were previously considered intractable. These include the mastery of large games like Go \citep{silver2016mastering} and Dota 2 \citep{berner2019dota}, as well as real-world applications ranging from healthcare \citep{pore2021safe}  to autonomous driving \citep{tai2017virtual} and robotics \citep{aractingi2023controlling}. However, despite these noteworthy advancements, even the most sophisticated DRL algorithms \citep{schulman2017proximal} face considerable challenges when analyzed on specific corner cases, where they persist in demonstrating a proclivity to commit critical mistakes \citep{corsi2024analyzing, szegedy2013intriguing}. These limitations present a threat to the reliability of DRL systems, particularly when deployed in safety-critical applications, where even a single failure can have potentially catastrophic consequences \citep{srinivasan2020learning, marvi2021safe, katz2019marabou, corsi2021formal}. 

Traditional techniques to address safety concerns aim to embed this aspect as part of the learning process; some examples include reward shaping \citep{tessler2018reward}, constrained reinforcement learning \citep{achiam2017constrained, ray2019benchmarking}, and adversarial training \citep{pinto2017robust}. While these approaches can significantly improve the general reliability of the policy, they often provide only empirical guarantees, and the benefits are often presented in expectation \citep{srinivasan2020learning, he2023autocost}. Although these may be sufficient for many problems, they cannot guarantee the safety of a system, which prevents their application in particularly safety-critical contexts.
% (e.g., where human life is involved). 

% % \vspace{-20pt}
% \begin{wrapfigure}{r}{0.56\textwidth}
% \vspace{-3pt}
% \centering
% \includegraphics[width=1.0\linewidth]{images/teaser.pdf} 
% \vspace{-30pt}
% \caption{In the offline process, the realizability check verifies whether the system is realizable, taking the system configuration as input, i.e., the dynamics of the environment, the safety requirements, and the input domain. If not realizable, the system needs to be changed. When proved to be realizable (i.e., a \propershield{}), the shield can be safely deployed in the environment for the online process.}
% \vspace{-5pt}
% \label{fig:intro:main}
% \end{wrapfigure}

\begin{figure}[t]
\centering
\includegraphics[width=0.7\linewidth]{images/teaser.pdf} 
\caption{In the offline process, the realizability check verifies whether the system is realizable, taking the system configuration as input, i.e., the dynamics of the environment, the safety requirements, and the input domain. If not realizable, the system needs to be changed. When proved to be realizable (i.e., a \propershield{}), the shield can be safely deployed in the environment for the online process.}
\label{fig:intro:main}
\vspace{-15pt}
\end{figure}

In contrast, a promising family of approaches provides formal safety guarantees through the adoption of an external component, commonly referred to as a shield \citep{garcia2015comprehensive, corsi2024verification}. In DRL, a shield acts as a protective wrapper over the agent to ensure that its actions remain within safe boundaries, effectively preventing it from making dangerous or undesired decisions. 
%
A shield is not an arbitrary program; it is essential that there are no instances where no available action satisfies all safety criteria simultaneously.
Otherwise, when the shielding mechanism encounters such scenarios, it fails to provide a safe action, leading to unsafe outcomes.

In this paper, we consider this crucial aspect of safety requirement satisfiability for all states. We define a \propershield{} as a shield that is always able to return an action that respects the given specifications for \textit{any} state of the system (a formal definition is presented as Def.~\ref{def:propershield}). 

In the logic community, ensuring this property is equivalent to guaranteeing the \realizability{} property for the shield (a formal definition is provided in section \ref{sec:preeliminaries}). 
However, it is particularly challenging for a human to provide a shield with safety requirements that it can always satisfy due to the compounding complexity of multiple safety requirements over continuous state and action spaces with many possible scenarios that can occur. 

% Thus to prevent deploying a shield with unrealizable safety requirements
To this end, we propose an approach that includes an automatic \realizability{} check as part of an offline procedure performed before deployment (an overview of the overall pipeline is provided in Fig.~\ref{fig:intro:main}). Intuitively, if the shield is not realizable, it means that the system cannot be safe in the required sense, and it is necessary to modify the dynamics of the system or relax the safety specifications. However, there is a scarcity of tools in the literature that support automatic realizability checking. A prominent example is the work of \citet{alshiekh2018safe}, which proposes to design a shield relying on the concept of Linear Temporal Logic (LTL). Their approach in particular allows the synthesis of the shield as a formal tool to automatically guarantee the \realizability{} of the system. However, this technique comes with a crucial limitation: the synthesizer for the LTL specifications is designed to handle only discrete states and actions. This constraint is overly restrictive for real-world reinforcement learning applications such as robotics where the state and action spaces are often continuous, high dimensional and nonlinear. 

This paper primarily builds upon the recent work on Realizability Modulo Theories of \citet{rodriguez2023boolean}. Applying their \realizability{} solver, we introduce a framework that for the first time is able to generate a \propershield{} capable of handling continuous state and action spaces. This significant advance enables to use shields in realistic domains that use data beyond Booleans.
%
To better understand the novelty of our method and its position in existing literature, Table \ref{tab:introduction:summary} presents a comparison with alternative techniques, highlighting the strengths of our approach compared to the baselines. 

In summary, the contributions of this paper are as follows: 
%
(1) First robotics application of shields verified from \textcolor{red}{LTLt specifications}.
% real-world application
%
(2) First \textcolor{red}{nonlinear} continuous shields.
%
(3) First study of the impact of the \textcolor{red}{correction optimization} in the policy: our approach allows us to use optimization techniques to return actions that are not only safe but also closely aligned with the original decisions proposed by the neural network. This ensures that the agent's behavior remains as optimal and effective as possible while adhering to safety constraints.
%
(4) Introduction of a \textcolor{red}{syntactic anticipation fragment of LTLt (and decidability proof)}, which allows us to incorporate robot dynamics directly into the safety requirements, allowing for a more accurate model-based representation of the physical world in which the agent's shield operates.  
% 
(5) Extensive empirical evaluation of our method: we demonstrate the effectiveness of our shielding approach in a mapless navigation domain, with additional experiments in a particle world multi-agent environment.
We demonstrate that our method can guarantee the realizability of safety requirements and ensure safety with continuous states and actions without compromising policy performance. 
%We formally prove that with our approach \realizability{} can be represented by a stateful shield,  which is crucial as it allows us to encode and enforce safety requirements that span multiple steps in the environment.

\begin{table*}[!t]
\centering
\begin{adjustbox}{width=1.0\linewidth,center}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
& \begin{tabular}[c]{@{}c@{}}Validate\\ Action\end{tabular} & \begin{tabular}[c]{@{}c@{}}Return Safe \\ Action\end{tabular} & \begin{tabular}[c]{@{}c@{}}Proper Shield \\ (Def.\ref{def:propershield})\end{tabular} & \begin{tabular}[c]{@{}c@{}}Optimization \\ Criteria\end{tabular} & \begin{tabular}[c]{@{}c@{}}Continuous \\ State Space\end{tabular} & \begin{tabular}[c]{@{}c@{}}Non- \\ Markovian\end{tabular} & Real Time             
\\ \hline
Na\"ive Conditions             & \cmark                                     & \xmark                                         & \xmark                                                                                  & \xmark                                            & \cmark                                             & \cmark & \cmark \\ 
\hline
Solver (e.g., Z3)                             & \cmark                                     & \cmark                                         & \xmark                                                                                  & \cmark                                            & \cmark                                             & \cmark & \xmark \\
\hline
\citet{alshiekh2018safe}         & \cmark                                     & \cmark                                         & \cmark                                                                                  & \xmark                                            & \xmark                                             & \xmark & \xmark \\ 
\hline
\citet{rodriguez2023boolean}         & \xmark                                     & \cmark                                         & \xmark                                                                                  & \xmark                                            & \cmark                                            & \xmark  & \xmark \\ 
\hline
This Work & \cmark                                     & \cmark                                         & \cmark                                                                                  & \cmark                                            & \cmark    & \cmark                                         & \xmark \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Comparison of different shielding techniques, highlighting the contribution of our method compared to existing works. 
% A na\"ive approach based on a sequence of conditions \textcolor{red}{(e.g., if/else statements)} can effectively limit the action space and prevent undesired direction, however, it cannot return a safe action (other than a default one, which is not always available). 
A na\"ive approach based on a sequence of conditions (e.g., if/else statements) can effectively constrain the action space and prevent undesired decisions, but it cannot return a safe action other than a default one (which is not always available).
A solver-based approach (e.g., Z3) can provide safe alternatives to unsafe actions, but it cannot guarantee the crucial \realizability{} property. This problem has been addressed in the work of \citet{alshiekh2018safe} but not in the case of continuous state and action spaces. Among all these approaches, our algorithm is the only one that can satisfy all these requirements. The last column highlights the remaining open problem of the computational time required to provide a safe alternative action.}
\label{tab:introduction:summary}
% \end{wraptable}
\vspace{-8pt}
\end{table*}


==> sections/method-bu.tex <==
% \newpage
\section{Realizable Continuous Shields with Non-Markovian Requirements}
\label{sec:method}

%%%%%% TODO: Check %%%%%%
% We applies a realizable shield to a robotic application with continuous state and action space.   % first?
% Non-markovian. Why important? and how important? How to achieve it? Implications in experiments.
% How connected to RL? - performance-wise, framework-wise
% two contributions: 1/ apply "realizable" "continuous"-space shield in robotics (encode dynamics, optimizer), 2/ non-markovian
%%%%%% Check %%%%%%

Our primary objective is to ensure safety in robotics tasks with continuous state and action spaces. % To achieve this, we implement a shield as an external component that wraps around the agent.  % adapt
We begin by introducing the foundational concept of a \propershield{}, which serves as the basis for our approach.
% Then, we extend a continuous-space proper shield
% show that a continuous-space proper shield is possible even with non-Markovian requirements, a crucial feature for enhancing performance in robotic applications.
% Then, we present a continuous-space shield that is realizable with non-Markovian requirements, a crucial feature for enhancing performance in robotic applications.
Then, we prove that a continuous-space shield can be ensured to be realizable with non-Markovian requirements, a crucial feature for enhancing performance in robotic applications.  % theoretic... prove?  % extend

% TODO: Check the review feedback.
% Make sure this is not tied with logic-based shield.  % avoid using realizability
\subsection{Proper Shield}
% A \propershield{} is a shield that ensures safety, providing safe alternatives to unsafe actions across \textit{all} states. In other words, if there exists even a single state where the shield fails to provide a safe action, it cannot be considered a proper shield.
A \propershield{} is a shield that can provide a safe alternative to unsafe actions across \textit{all} the states of the system given a set of safety constraints $\varphi$. In other words, if there exists even a single state where the shield fails to provide a safe action, it cannot be considered proper. We instantiate our proper shield as a stateful component, where the shield's state $h \in H$ is defined as the sequence of the constraints that held in previous timesteps of an episode.
\textcolor{red}{Since the number of constraints is finite, the shield effectively uses stateful memory.} % \textcolor{red}{Note that the amount of constraints is finite, thus a shield uses stateful memory.}
By construction, $h \in H$ consists of safe states (i.e., $\varphi$ has not been violated so far); otherwise, this would contradict the specification.  %  for $\varphi$
% The shield takes as input an action $a \in A$, an observation $o \in O$, and a shield state $h \in H$, while $\varphi$ denotes the specification (e.g., a safety specification). Then: 
More formally, given an action $a \in A$, an observation $o \in O$, a shield state $h \in H$, and a set of specification $\varphi$, we define a proper shield as: 

% TODO: connect with non-markovian?
% TODO: % a broad concept: not tied with LTL / can be non-markovian / can be discrete   - does not need to be LTL based, may or may not have a history, discrete or continuous
\begin{definition}[\propershield{}]
\label{def:propershield} 
{\ \\}
\fbox{\begin{minipage}{1.0\textwidth}
A \propershield{} is a function $\zeta: A \times O \times H \to A$, such that $\forall$ \( o \in O \) and \( h \in H \), $\varphi(\zeta(a, o, h),o, h)$ holds.
\end{minipage}}
\end{definition}
\jb{(I was confused reading the 2nd paragraph of 3.1, and I think it would have been clearer if we lead with definition 1 (maybe just say it inline without fancy formatting.) and then explained what a, o, and h is. Leading with h confused me since I didn't yet even know explicitly what a shield was or what a "specification" was.
Additionally, let's define a shield's state $h$ as its history early on and then refer to $h$ as shield "history" from then on to not confuse shield states with environment states. Finally, why do we need $h$? I don't think it's explained.)}

Intuitively, a \propershield{} is a function $\zeta$ designed to always return an action $a$ such that $\varphi$ holds when starting from the initial state.
The shield $\zeta$ is combined with an external agent $\pi$ (in our case, an RL agent) to ensure that the composition \textcolor{red}{$\zeta \cdot \pi$} never violates $\varphi$. 
% in the context of RL... online shielding process
At each timestep, given the shield's history $h$: (1) $\pi$ receives observation inputs $o$ from the environment and produces an action $a$; (2) we check whether $\varphi(a, o, h)$ holds; and (3) if $\varphi(a, o, h)$ holds, the shield does not intervene, but if there is a violation, it overrides $a$ with a corrected action $\hat{a} = \zeta (a,o,h)$ such that  $\varphi(\hat{a},o,h)$ now holds for that step, as described in Fig.~\ref{fig:intro:main}.

% While we build our shield on reactive synthesis, this definition is not tied to a specific method.  % TODO: say shield can be implemented with different ways. Note that shield is a general concept. There are many ways of implementing it. % also, discrete and continuous 
% builds on powerful theories in logic.
While shields can be constructed using various frameworks (see Tab.~\ref{tab:introduction:summary}), our approach builds on powerful tools in logic.  %  to constructing a proper shield  % theories
Specifically, we design a temporal specification $\varphi$ that describes the desired safety requirements.
We then \textcolor{red}{check whether $\varphi$ is realizable}. A positive result implies that $\zeta$ exists.
Although $\zeta$ can be automatically obtained by applying reactive synthesis to $\varphi$ [\textcolor{red}{cite}], we choose to construct $\zeta$ manually to maintain code interpretability.
\jb{Maybe say here that "We implement our shield and specification using xyz specific code framework from xyz work (cite)."}
% where we can apply reactive synthesis to $\varphi$ [\textcolor{red}{cite}] to automatically obtain $\zeta$.  % either
%
%By designing a realizable specification $\varphi$ and applying reactive synthesis to it, we derive a safe strategy $\zeta$, which serve as a proper shield by construction.  % will always   % is equivalent to  % specifically,   % A proper shield represents the safe strategy $\zeta$ for a realizable specification $\varphi$. This means that the shield provides safe alternatives to any unsafe actions in all states.
% Ensuring that the specification $\varphi$ is realizable is essential as an unrealizable specification may lead to an unsatisfiable (\unsat{}) result, indicating that no safe action is possible in the given state.

Ensuring that $\varphi$ is realizable is essential, as unrealizability could lead to situations where no safe action is possible for a given state.
In such cases, computing $\hat{a}$ is not possible because the formula is unsatisfiable (\unsat{}).
%
In our framework (see Fig.~\ref{fig:intro:main}, left), we check the realizability of $\varphi$ as part of an offline process prior to deployment, treating the observation $o$ and shield state $h$ as uncontrollable variables, while considering the action $a$ as a controllable variable.  % To do so  % in the process  % Bridging components in RL with the concepts from logic,  % Describe how? in the later section?

\citet{alshiekh2018safe} showed that a proper shield can be constructed using LTL, but their approach is limited to discrete state and action spaces.
This restricts its applicability to robotics tasks and fails to capture accurate environment dynamics.
In contrast, our shield leverages the more expressive specification language, LTLt, enabling the construction of a continuous-space proper shield that incorporates accurate dynamics directly into the specification.
%
% Moreover, since the continuous domain is a metric space, we can measure how \textit{far} the correction $\hat{a}$ is from the original candidate output $a$. This allows us to optimize the shield's safe-action correction by returning $\hat{a}$ such that it is the closest safe value to the agent's proposed action $a$.
Moreover, since the continuous domain is a continuous space, we can minimize a distance metric between the correction $\hat{a}$ and the original candidate output $a$. This allows us to optimize the shield's safe-action correction by returning $\hat{a}$ such that it is the closest safe value to the agent's proposed action $a$.

%%%%%
% \citet{alshiekh2018safe} showed that a proper shield can be constructed using LTL, but their approach is limited to discrete state and action spaces, restricting its applicability in robotics tasks and failing to capture accurate environment dynamics.
% In contrast, our shield leverages a more advanced tool called LTLt, enabling the construction of a continuous-space proper shield.  % 
% This approach not only ensures safety but also encodes accurate dynamics as part of the specification.
% Since the continuous domain is a metric space, we can measure how far the correction is from the original candidate output. Therefore, we can also optimize the shield's safe-action correction by returning the safe value closest to the agent's proposed action.
%%%%%

% Shorten
\subsection{Non-Markovian Encoding in LTLt} \label{subsec:nonMarkov}

We can check realizability of proper shields that encode markovian properties:

\begin{example}
    Consider a robot moving in a two-coordinates scenario whose position is received by sensors $x$ and $y$. The robot moves via actuators $d$ and $\theta$ by which, in every timestep, it selects the desired distance and angle respectively.
    %
    In addition, the scenario has a concrete region $r=[(0.0,0.5), (0.0, 0.5)]$ such that, if the robot visits $r$, it has to choose values for the variables it controls ($d$ and $\theta$) such that the robot is out of $r$ in the next timestep.
    %
    We can encode this safety property in LTLt easily:
    $$[(0.0 \leq x \leq 0.5) \wedge (0.0 \leq x \leq 0.5)] \rightarrow \neg[(0.0 \leq \cos(\theta)\cdot d \leq 0.5) \wedge (0.0 \leq \sin(\theta)\cdot d \leq 0.5)]$$
\end{example}

%
Often, these properties are enough to avoid collisions.
%
However, using these properties might make our policy to become too conservative and have an impact in our performance (e.g., success rate). 
%
Thus,  we are also interested in encoding multistep properties (which may require bounded memory) such as: do not repeat the action. Thanks to this, we avoid loops and enhance performance.

%
We now show how to encode non-Markovian requirements in a decidable fragment of LTLt.
%
\begin{example} \label{ex:nonMarkovian}
Consider a robot moving between a set of regions R, where each $r \in R$ is defined by $(x,y)$ coordinates. For instance, $r_0=[(0.0,0.5), (0.0, 0.5)]$ means that the region $r_0$ goes from $0.0$ to $0.5$ in the $x$ axis and in the $y$ axis. Also, we denote with $r^x_l$ and $r^y_l$ the lower bound of the region in the $x$ and $y$ axes (i.e., $0.0$ in both cases), and with $r^x_u$ and $r^y_u$ the upper bound of the region in the $x$ and $y$ axes (i.e., $0.5$ in both cases)
%
Now, we specify a non-Markovian behaviour: 

``If the robot is in region $r \in R$, then it cannot visit $r$ again in at least $i$ timesteps."

Let $\theta$ and $d$ correspond to the angle and distance decided by the system.
%
We now formally state our non-Markovian property using an LTLt formula $\varphi = A \rightarrow G$, where $A$ represents the assumptions, and $G$ specifies the guarantees the system must uphold under those assumptions:

\begin{minipage}{.5\linewidth}
\begin{align*}
    \square [(x = & \lhd \cos(\theta) \cdot \lhd d + \lhd x) \\ & \wedge (y = \lhd \sin(\theta) \cdot \lhd d + \lhd y )]
\end{align*}
\end{minipage}
%
\begin{minipage}{.5\linewidth}
\begin{align*}
    \square & [\bigwedge_{r\in R} [(r_l^x \leq x \leq r_u^x) \wedge (r_l^y \leq y \leq r_u^y)] \\
    \rightarrow & \square_{[1,i]}\neg [(r_l^x \leq x \leq r_u^x) \wedge (r_l^y \leq y \leq r_u^y)]],
\end{align*}
\end{minipage}\\

where: \jb{This example is still unreadable, and I don't think any small change will fix this. Either remove this example entirely or come up with a new example that is specifically optimized for the readability of the LTLt formula.)}

\begin{itemize}
    \item $A$ (left) is an environment assumption that describes the dynamics of $(x,y)$; i.e., in this case the fact that the values of $x$ and $y$ are given by the previous values of $\theta$, $d$ and $x$ or $y$.
    % The operator $\lhd x$ allows access to the value of x from the previous timestep.
    The operator $\lhd x$ represents a specific value that the variable x has taken in previous timesteps.
    \item $G$ (right) are the guarantees by the system, in this case, stating that if $(x,y)\in r$ in a given timestep, then $(x,y)\notin r$ throughout $i$ timesteps; i.e., $r$ will not be re-visited for $i$ timesteps.
\end{itemize}

%
% This requirement is a powerful non-markovian and can be used in many cases. Howoever, it is not decidable because it is encoded in a fragement of LTLt stemming from the usage of $\lhd$.
Note how it is very natural to use $\lhd$ to define $\varphi$.
%
However, $\varphi$ is encoded in a fragment of LTLt that is not decidable due to the operator $\lhd$.
This operator introduces unbounded memory to the program \textcolor{red}{via the uncontrolled infinite nesting of the operator which at the same time may end up in the infinite recursion.} \footnote{Find more information in the supplementary material}.
Thus, realizability checking is not guaranteed to terminate and we need to rewrite $A$ without $\lhd$ in an LTLt formula as follows:
 % $\varphi' = A' \rightarrow G'$
% intuition

% \begin{minipage}{.5\linewidth}
\begin{align*}
    \square[\bigwedge_{r \in R}  [(r^{x}_l \leq \cos(\theta)\cdot d +x \leq r^{x}_u) \\ \wedge (r^{y}_l \leq \sin(\theta)\cdot d +y \leq r^{y}_u)]  
    \\ \rightarrow \ocircle  [(r^{x}_l \leq x \leq r^{x}_u) \wedge (r^{y}_l \leq y \leq r^{y}_u)]],
\end{align*}
% \end{minipage}
%
% \begin{minipage}{.5\linewidth}
% \begin{align*}
%     \square [\bigwedge_{r \in R} [[(r^{x}_l \leq \cos(\theta)\cdot d +x \leq r^{x}_u) \wedge \\ (r^{y}_l \leq \sin(\theta)\cdot d +y \leq r^{y}_u)] \\ 
%     \rightarrow \square_{[1,i]}\neg [(r^{x}_l \leq \cos(\theta)\cdot d +x \leq r^{x}_u) \\ \wedge (r^{y}_l \leq \sin(\theta)\cdot d +y \leq r^{y}_u)]]],
% \end{align*}
% \end{minipage}\\

\noindent which means that whenever the predicted $(x, y)$ location, based on the dynamics and the values of $x,y,\theta,$ and $d$ at timestep $k$, lies in $r$, then $(x,y)$ at timestep $k+1$ is necessarily in $r$.  %  instantiations  %  (i.e., $(\cos(\theta)\cdot d +x, \sin(\theta)\cdot d +y)$)
% \noindent which means that whenever $\theta$, $d$ and $(x,y)$ are in $r$ at timestep $k$, then $(x,y)$ at timestep $k+1$ is necessarily in $r$.  %  instantiations
The guarantee ($G$) remains unchanged.
% \noindent Intuitively, $A'$ (left) in $\varphi'$ means that there whenever $\theta$ and $d$ and $(x,y)$ are in $r$ instantiations at timestep $k$, then $(x,y)$ instantiations at timestep $k+1$ is necessarily in $r$.
%
% Also, $G'$ (right) means that, if $\theta$ and $d$ are in $r$ in timestep $k$, then throught $i$ timesteps, $\theta$ and $d$ must be chosen so that they are not in $r$..
\end{example}

%An essential observation that makes this transformation possible is that we are assuming no uncertainty in our domain. In particular, each valuation of $(a^0, a^1)$ in state $(x,y,r)$ induces a very precise $(x',y',r')$ in the next timestep: i.e., we can perfectly \textit{anticipate} the next state of the environment given a movement of the system and current state. Thus, we can \textit{anticipate} the dangerous movement of the system, and override it.
An essential observation that makes this transformation possible is that we are assuming to have access to a safety-relevant subset of the robot's dynamic, often called \textit{safety-dynamics} in the literature \citep{yang2023safe}. In our example, each valuation of $(\theta, d)$ in state $(x,y,r)$ allows to compute $(x',y',r')$ in the next timestep: i.e., we can \textit{anticipate} the safety-relevant components of the next state given the action and the current state of the system. Thus, we can \textit{anticipate} any unsafe action of the agent, and potentially override it.

% \begin{definition}
% \label{def:method:anticipation-fragment}
%     If $\varphi$ is an LTLt formula for which the next value of the environment variables can be fully determined from the current environment values and system values, then $\varphi$ can be rewritten in $\lhd$.
%     %
%     Thus, realizability for such $\varphi$ is decidable.
%     \textcolor{red}{Add a definition of anticipation fragment - use the term anticipation fragment - as we mentioned in introduction.}
% \end{definition}
\begin{theorem}
\label{thm:anticipation} 
    If $\varphi$ is an LTLt formula for which the next value of the environment variables can be fully determined from the current environment values and system values, then $\varphi$ can be rewritten without making use of $\lhd$.
\end{theorem}

\begin{definition}
\label{def:method:anticipation-fragment} 
    The class of LTLt formula that can be translated to not using $\lhd$ is called the anticipation fragment of LTLt.
\end{definition}

\begin{corollary}
\label{thm:anticipation} 
    If $\varphi$ belongs to the ancitipation fragment, then realizability of $\varphi$ is decidable.
\end{corollary}

% Completely characterizing the exact class of specifications that can be rewritten without $\lhd$ is future work. Moreover, \textcolor{red}{it is unclear how this works with POMDPs (i.e., without perfect anticipation)}.
\noindent Note that we leave a complete characterization of the \textit{anticipation fragment class} as a future work, however, following from Def.~\ref{def:method:anticipation-fragment} we can ensure that our robotic navigation problem belongs to this class. You can find details such as proof for Thm.~\ref{thm:anticipation} in Appendix.



% \subsection{Architecture Overview}

% In this paper we show how to use \textit{shield-synthesis}, where reactive synthesis computes a shield $\zeta$ from $\varphi$ (in LTL modulo real arithmetic, i.e., continuous domains) and $\zeta$ is combined with an external agent $\pi$ (in our case, an RL-trained agent) to ensure that the composition $\pi \cdot \zeta$ will never violate $\varphi$. 
% %
% In each timestep, given the shield history $h$: (1) $\pi$ receives observation inputs $o$ from the environment and produces action outputs $a$; (2) $\zeta$ checks whether $\varphi(a, o, h)$ holds; and (3) if $\varphi(a, o, h)$ holds, the shield does not intervene, whereas in case of a violation, it overrides $a$ with a correction $\hat{a} = \zeta (a,o,h)$ such that  $\varphi(\hat{a},o,h)$ now holds in that step.
% %

% This online process translates to providing a valid action (i.e., the assignment of the variables controlled by the system) that satisfies the specified requirements given the current state of the environment. The shield will propagate the continuous constraints through time and will check if the agent's action satisfies all requirements and otherwise provide an alternative safe action. In LTLt, this is done by performing a query to a constraint satisfaction solver. If the constraint specification is not realizable, the shield may return an unsatisfiable (\unsat{}) result, indicating that no safe action is possible given the current state.

% In our framework (see Fig.~\ref{fig:intro:main}(left)) we first check offline whether $\varphi$ is realizable, which ensures that for any possible state of the environment, the shield can always return a safe action.
% %
% Moreover, since the continuous domain is a metric space, we can measure how far the correction is from the original candidate output. Therefore, we can also optimize the shield's safe-action correction by returning the safe value closest to the agent's proposed action.
